Efficient Feature Extraction for High-resolution Video Frame Interpolation

Most deep learning methods for video frame interpolation consist of three main components: feature extraction, motion estimation, and image synthesis. Existing approaches are mainly distinguishable in terms of how these modules are designed. However, when interpolating high-resolution images, e.g. at 4K, the design choices for achieving high accuracy within reasonable memory requirements are limited. The feature extraction layers help to compress the input and extract relevant information for the latter stages, such as motion estimation. However, these layers are often costly in parameters, computation time, and memory. We show how ideas from dimensionality reduction combined with a lightweight optimization can be used to compress the input representation while keeping the extracted information suitable for frame interpolation. Further, we require neither a pretrained flow network nor a synthesis network, additionally reducing the number of trainable parameters and required memory. When evaluating on three 4K benchmarks, we achieve state-of-the-art image quality among the methods without pretrained flow while having the lowest network complexity and memory requirements overall.

==> figures_tables/finetuned.tex <==
\begin{figure}[t]
    \centering
    \subfigure[Original PCA]{
    \begin{minipage}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/temp_picdown_small.png}
    \end{minipage}
    \label{fig:originalPCA}
    }
    \hspace{5pt}
    \subfigure[With finetuning]{
    \begin{minipage}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/test_small.png}
        \label{fig:finetuned}
    \end{minipage}
    }
    \caption{Image reconstruction with a fraction of the projections directions.
    }
    \label{fig:finetuned}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
